Real-Time Adaptive Image Compression

We present a machine learning-based approach to lossy image compression which outperforms all existing codecs, while running in real-time. Our algorithm typically produces files 2.5 times smaller than JPEG and JPEG 2000, 2 times smaller than WebP, and 1.7 times smaller than BPG on datasets of generic images across all quality levels. At the same time, our codec is designed to be lightweight and deployable: for example, it can encode or decode the Kodak dataset in around 10ms per image on GPU. Our architecture is an autoencoder featuring pyramidal analysis, an adaptive coding module, and regularization of the expected codelength. We also supplement our approach with adversarial training specialized towards use in a compression setting: this enables us to produce visually pleasing reconstructions for very low bitrates.

==> discussion.tex <==
% !TEX root = main.tex

\vspace{-0.1in}
\section{Conclusion}

In this work, we introduced a new approach for image compression, which outperforms all other techniques and is computationally efficient. We believe, however, that our work only scratches the surface, and that there are many important and exciting problems to be tackled in the domain of image compression. 


